Directional variograms for multivariate extremes

Multivariate generalized Pareto distributions arise as limits of threshold exceedances and form a central model class for multivariate extremes. Existing inference methods based on the extremal variogram condition on the value of a single component, which can be statistically suboptimal. We generalize this approach by conditioning the multivariate generalized Pareto random vector $Y$ to lie on arbitrary half-spaces. Specifically, for a direction vector $v$, we introduce the random vector $Y^v = (Y \mid v^\top Y > 0)$ and define the associated $v$-variogram $\Gamma_{ij}^v=\mathrm{Var}(Y_i^v-Y_j^v)$. We establish the decomposition $Y^v \stackrel{d}{=} W^v+E\mathbf{1}$ into the so-called $v$-extremal function $W^v$ and an independent exponential random variable $E$, and derive several results relating these random variables to each other. For logistic, Dirichlet, and H\"usler-Reiss multivariate generalized Pareto models, we derive closed-form expressions for $\Gamma^v$. In the H\"usler-Reiss case, we further derive new density representations and identify a distinguished resistance-curvature vector $v_0$ that uniquely centers the Gaussian law of $W^{v_0}$ while characterizing the least-mass half-space. On the statistical side, we introduce empirical $v$-variograms and show in a simulation study that the choice of $v$ induces a pronounced bias-variance trade-off that is strongly related to the mass of the conditioning half-space. Moreover, combining information across multiple directions $v$ can substantially reduce estimation variance relative to methods based on a single vector.

==> tikzR/densityProjections/OneVec.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-60.70,215.56) -- (-59.46,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-55.59,210.45) -- (-49.23,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-50.48,205.34) -- (-39.01,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-45.37,200.23) -- (-28.79,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-40.26,195.12) -- (-18.57,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-35.15,190.01) -- ( -8.35,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-30.04,184.90) -- (  1.87,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-24.93,179.79) -- ( 12.09,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-19.82,174.68) -- ( 22.31,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-14.71,169.57) -- ( 32.53,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( -9.60,164.46) -- ( 42.75,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( -4.49,159.35) -- ( 52.97,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.62,154.24) -- ( 63.19,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  5.73,149.13) -- ( 73.41,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 10.84,144.02) -- ( 83.63,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 15.95,138.91) -- ( 93.85,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 21.06,133.80) -- (104.07,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 26.17,128.69) -- (114.29,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 31.28,123.58) -- (124.51,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 36.39,118.47) -- (134.73,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 41.50,113.36) -- (144.96,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 46.61,108.25) -- (155.18,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 51.73,103.14) -- (165.40,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 56.84, 98.03) -- (175.62,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 92.92) -- (185.84,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 67.06, 87.81) -- (196.06,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.17, 82.70) -- (206.28,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 77.28, 77.59) -- (216.50,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 82.39, 72.48) -- (216.81,206.90);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 87.50, 67.37) -- (216.81,196.68);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 92.61, 62.26) -- (216.81,186.46);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 97.72, 57.15) -- (216.81,176.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.83, 52.04) -- (216.81,166.02);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (107.94, 46.93) -- (216.81,155.80);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (113.05, 41.82) -- (216.81,145.58);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (118.16, 36.71) -- (216.81,135.36);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (123.27, 31.60) -- (216.81,125.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (128.38, 26.49) -- (216.81,114.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (133.49, 21.37) -- (216.81,104.70);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (138.60, 16.26) -- (216.81, 94.48);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (143.71, 11.15) -- (216.81, 84.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (148.82,  6.04) -- (216.81, 74.03);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (153.93,  0.93) -- (216.81, 63.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (159.04, -4.18) -- (216.81, 53.59);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (164.15, -9.29) -- (216.81, 43.37);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (169.26,-14.40) -- (216.81, 33.15);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (174.37,-19.51) -- (216.81, 22.93);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (179.48,-24.62) -- (216.81, 12.71);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (184.59,-29.73) -- (216.81,  2.49);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (189.70,-34.84) -- (216.81, -7.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (194.81,-39.95) -- (216.81,-17.95);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (199.92,-45.06) -- (216.81,-28.17);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (205.03,-50.17) -- (216.81,-38.39);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (210.14,-55.28) -- (216.81,-48.61);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (215.25,-60.39) -- (216.81,-58.83);

\path[] ( 61.95, 92.92) --
	(216.81,-61.95) --
	(216.81,216.81) --
	(-61.95,216.81) --
	( 61.95, 92.92) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 92.92) -- (216.81, 92.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 91.11) --
	(216.81, 92.92) --
	(213.68, 94.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,  0.00) -- ( 61.95,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 63.75,213.68) --
	( 61.95,216.81) --
	( 60.14,213.68);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 61.95, 92.92) -- ( 77.43,108.41);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 77.28,108.25) -- ( 77.43,108.41);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 75.94,102.82) --
	( 77.43,108.41) --
	( 71.85,106.91);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 83.43,106.11) {$\mathbf{1}/2$};

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (  0.00,154.86) -- (216.81,-61.95);
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 92.92) -- ( 92.92, 61.95);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 85.94, 63.82) --
	( 92.92, 61.95) --
	( 91.05, 68.93);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 92.92, 61.95) -- (185.84,154.86);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (183.97,147.88) --
	(185.84,154.86) --
	(178.86,152.99);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (185.84,154.86) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 85.18, 75.69) {$W^{\mathbf{1}}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.96,124.69) {$E \cdot \mathbf{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (185.84,160.86) {$Y^{\mathbf{1}}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.07, 81.18) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 67.95,204.60) {$\mathbb{R}$};
\end{scope}
\end{tikzpicture}


==> tikzR/densityProjections/V_onePerp.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-183.35,215.56) -- (-182.10,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-176.53,212.16) -- (-171.88,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-169.72,208.75) -- (-161.66,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-162.91,205.34) -- (-151.44,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-156.09,201.94) -- (-141.22,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-149.28,198.53) -- (-131.00,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-142.46,195.12) -- (-120.78,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-135.65,191.72) -- (-110.56,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-128.84,188.31) -- (-100.34,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-122.02,184.90) -- (-90.12,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-115.21,181.50) -- (-79.90,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-108.40,178.09) -- (-69.68,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-101.58,174.68) -- (-59.46,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-94.77,171.28) -- (-49.23,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-87.96,167.87) -- (-39.01,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-81.14,164.46) -- (-28.79,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-74.33,161.06) -- (-18.57,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-67.51,157.65) -- ( -8.35,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-60.70,154.24) -- (  1.87,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-53.89,150.83) -- ( 12.09,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-47.07,147.43) -- ( 22.31,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-40.26,144.02) -- ( 32.53,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-33.45,140.61) -- ( 42.75,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-26.63,137.21) -- ( 52.97,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-19.82,133.80) -- ( 63.19,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (-13.00,130.39) -- ( 73.41,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( -6.19,126.99) -- ( 83.63,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.62,123.58) -- ( 93.85,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  7.44,120.17) -- (104.07,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 14.25,116.77) -- (114.29,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 21.06,113.36) -- (124.51,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 27.88,109.95) -- (134.73,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 34.69,106.55) -- (144.96,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 41.50,103.14) -- (155.18,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 48.32, 99.73) -- (165.40,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 55.13, 96.33) -- (175.62,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 92.92) -- (185.84,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 68.76, 89.51) -- (196.06,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 75.57, 86.10) -- (206.28,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 82.39, 82.70) -- (216.50,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 89.20, 79.29) -- (218.05,208.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 96.01, 75.88) -- (219.33,199.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.83, 72.48) -- (220.60,190.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (109.64, 69.07) -- (221.88,181.31);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (116.46, 65.66) -- (223.16,172.37);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (123.27, 62.26) -- (224.44,163.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (130.08, 58.85) -- (225.71,154.48);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (136.90, 55.44) -- (226.99,145.54);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (143.71, 52.04) -- (228.27,136.60);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (150.52, 48.63) -- (229.55,127.65);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (157.34, 45.22) -- (230.82,118.71);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (164.15, 41.82) -- (232.10,109.77);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (170.96, 38.41) -- (233.38,100.82);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (177.78, 35.00) -- (234.66, 91.88);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (184.59, 31.60) -- (235.93, 82.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (191.41, 28.19) -- (237.21, 74.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (198.22, 24.78) -- (238.49, 65.05);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (205.03, 21.37) -- (239.77, 56.11);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (211.85, 17.97) -- (241.04, 47.17);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (218.66, 14.56) -- (242.32, 38.22);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (225.47, 11.15) -- (243.60, 29.28);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (232.29,  7.75) -- (244.88, 20.34);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (239.10,  4.34) -- (246.16, 11.39);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (245.92,  0.93) -- (247.43,  2.45);

\path[] ( 61.95, 92.92) --
	(247.78,  0.00) --
	(216.81,216.81) --
	(-185.84,216.81) --
	( 61.95, 92.92) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 92.92) -- (216.81, 92.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 91.11) --
	(216.81, 92.92) --
	(213.68, 94.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,  0.00) -- ( 61.95,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 63.75,213.68) --
	( 61.95,216.81) --
	( 60.14,213.68);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 61.95, 92.92) -- ( 72.27,113.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.17,113.36) -- ( 72.27,113.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.62,107.80) --
	( 72.27,113.57) --
	( 67.45,110.38);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 72.27,119.57) {$v$};

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (  0.00,123.89) -- (216.81, 15.49);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (  0.00,154.86) -- (216.81,-61.95);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 61.95, 92.92) -- ( 92.92,123.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 92.61,123.58) -- ( 92.92,123.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 91.42,118.31) --
	( 92.92,123.89) --
	( 87.33,122.40);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 98.92,121.60) {$\mathbf{1}$};

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (108.41, 46.46) -- (123.89, 61.95);
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 92.92) -- (123.89, 61.95);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (116.68, 61.51) --
	(123.89, 61.95) --
	(119.91, 67.98);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (123.89, 61.95) -- (201.32,139.38);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (199.45,132.40) --
	(201.32,139.38) --
	(194.34,137.51);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (201.32,139.38) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (108.41, 75.69) {$W^{v}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (184.09,113.85) {$E \cdot \mathbf{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.32,145.38) {$Y^{v}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.07, 81.18) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 67.95,204.60) {$\mathbb{R}$};
\end{scope}
\end{tikzpicture}


==> tikzR/densityProjections/e1.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,215.56) -- ( 63.19,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,205.34) -- ( 73.41,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,195.12) -- ( 83.63,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,184.90) -- ( 93.85,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,174.68) -- (104.07,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,164.46) -- (114.29,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,154.24) -- (124.51,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,144.02) -- (134.73,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,133.80) -- (144.96,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,123.58) -- (155.18,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,113.36) -- (165.40,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,103.14) -- (175.62,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 92.92) -- (185.84,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 82.70) -- (196.06,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 72.48) -- (206.28,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 62.26) -- (216.50,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 52.04) -- (216.81,206.90);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 41.82) -- (216.81,196.68);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 31.60) -- (216.81,186.46);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 21.37) -- (216.81,176.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95, 11.15) -- (216.81,166.02);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,  0.93) -- (216.81,155.80);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 71.23,  0.00) -- (216.81,145.58);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 81.45,  0.00) -- (216.81,135.36);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 91.67,  0.00) -- (216.81,125.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (101.89,  0.00) -- (216.81,114.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (112.11,  0.00) -- (216.81,104.70);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (122.33,  0.00) -- (216.81, 94.48);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (132.56,  0.00) -- (216.81, 84.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (142.78,  0.00) -- (216.81, 74.03);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (153.00,  0.00) -- (216.81, 63.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (163.22,  0.00) -- (216.81, 53.59);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (173.44,  0.00) -- (216.81, 43.37);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (183.66,  0.00) -- (216.81, 33.15);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (193.88,  0.00) -- (216.81, 22.93);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (204.10,  0.00) -- (216.81, 12.71);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (214.32,  0.00) -- (216.81,  2.49);

\path[] ( 61.95,  0.00) --
	(216.81,  0.00) --
	(216.81,216.81) --
	( 61.95,216.81) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 92.92) -- (216.81, 92.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 91.11) --
	(216.81, 92.92) --
	(213.68, 94.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,  0.00) -- ( 61.95,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 63.75,213.68) --
	( 61.95,216.81) --
	( 60.14,213.68);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 61.95,  0.00) -- ( 61.95,216.81);
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 92.92) -- ( 61.95, 30.97);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 58.33, 37.23) --
	( 61.95, 30.97) --
	( 65.56, 37.23);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 30.97) -- (185.84,154.86);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (183.97,147.88) --
	(185.84,154.86) --
	(178.86,152.99);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (185.84,154.86) circle (  2.25);

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 55.95, 44.16) {$W^{e_1}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (154.67,115.40) {$E \cdot \mathbf{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (185.84,160.86) {$Y^{e_1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.07, 81.18) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 67.95,204.60) {$\mathbb{R}$};
\end{scope}
\end{tikzpicture}


==> tikzR/graphs/G_03_graph.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (144.54,144.54);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 66.10,124.29) -- ( 20.25, 78.44);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 78.44,124.29) -- (124.29, 78.44);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 20.25, 66.10) -- ( 66.10, 20.25);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 22.81, 72.27) -- (121.73, 72.27);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,130.46) circle (  8.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 14.08, 72.27) circle (  8.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27, 14.08) circle (  8.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (130.46, 72.27) circle (  8.73);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at ( 72.27,126.61) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at ( 14.08, 68.42) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at ( 72.27, 10.23) {3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at (130.46, 68.42) {4};
\end{scope}
\end{tikzpicture}


==> tikzR/rowVectors/gamma_sigmaii_sigmaij.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 72.27) -- (216.81, 72.27);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 70.46) --
	(216.81, 72.27) --
	(213.68, 74.08);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,  0.00) -- ( 72.27,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.08,213.68) --
	( 72.27,216.81) --
	( 70.46,213.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.58, 60.53) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 78.27,202.95) {$\mathbb{R}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (169.83, 97.56) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (180.67,144.54) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (126.47,180.67) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (169.83, 85.83) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (186.67,142.24) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (126.47,186.67) {3};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (169.83, 97.56) --
	(180.67,144.54);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (181.25,118.76) {$\Gamma_{12}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27, 72.27) --
	(169.83, 97.56);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (130.81, 75.71) {$\Sigma_{11}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27, 72.27) --
	(107.25, 81.34) --
	(107.14, 81.74) --
	(107.03, 82.14) --
	(106.91, 82.54) --
	(106.79, 82.94) --
	(106.67, 83.34) --
	(106.54, 83.73) --
	(106.40, 84.13) --
	(106.26, 84.52) --
	(106.12, 84.91) --
	(105.97, 85.30) --
	(105.82, 85.69) --
	(105.66, 86.08) --
	(105.50, 86.46) --
	(105.34, 86.84) --
	(105.17, 87.22) --
	(104.99, 87.60) --
	(104.81, 87.98) --
	(104.63, 88.35) --
	(104.44, 88.72) --
	(104.25, 89.09) --
	(104.05, 89.46) --
	(103.85, 89.83) --
	(103.65, 90.19) --
	(103.44, 90.55) --
	(103.23, 90.91) --
	(103.01, 91.26) --
	(102.79, 91.62) --
	(102.57, 91.97) --
	(102.34, 92.31);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 95.36, 80.10) {$\Sigma_{12}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (180.67,144.54) --
	(126.47,180.67);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (153.57,168.61) {$\Gamma_{23}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27, 72.27) --
	(180.67,144.54);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (115.63,107.18) {$\Sigma_{22}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27, 72.27) --
	(102.34, 92.31) --
	(101.97, 92.85) --
	(101.60, 93.38) --
	(101.22, 93.90) --
	(100.83, 94.41) --
	(100.42, 94.92) --
	(100.01, 95.42) --
	( 99.60, 95.91) --
	( 99.17, 96.40) --
	( 98.73, 96.88) --
	( 98.29, 97.35) --
	( 97.83, 97.81) --
	( 97.37, 98.26) --
	( 96.90, 98.71) --
	( 96.43, 99.14) --
	( 95.94, 99.57) --
	( 95.45, 99.99) --
	( 94.95,100.40) --
	( 94.44,100.80) --
	( 93.93,101.20) --
	( 93.41,101.58) --
	( 92.88,101.95) --
	( 92.34,102.32) --
	( 91.80,102.67) --
	( 91.25,103.02) --
	( 90.70,103.35) --
	( 90.14,103.68) --
	( 89.58,103.99) --
	( 89.01,104.30) --
	( 88.43,104.59);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 89.01, 88.73) {$\Sigma_{23}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (126.47,180.67) --
	(169.83, 97.56);

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  1.00] at (142.15,136.82) {$\Gamma_{31}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27, 72.27) --
	(126.47,180.67);

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 93.37,124.18) {$\Sigma_{33}$};
\end{scope}
\end{tikzpicture}


==> tikzR/rowVectors/shift_circumhyper.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 72.27) -- (216.81, 72.27);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 70.46) --
	(216.81, 72.27) --
	(213.68, 74.08);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,  0.00) -- ( 72.27,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.08,213.68) --
	( 72.27,216.81) --
	( 70.46,213.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.58, 60.53) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 78.27,202.95) {$\mathbb{R}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (109.65, 38.91) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (120.49, 85.88) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 66.29,122.02) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (109.65, 27.17) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (126.49, 83.59) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 66.29,128.02) {3};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (109.65, 38.91) --
	(120.49, 85.88);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (120.49, 85.88) --
	( 66.29,122.02);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 66.29,122.02) --
	(109.65, 38.91);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (122.37, 72.27) --
	(122.27, 75.45) --
	(121.97, 78.61) --
	(121.47, 81.75) --
	(120.77, 84.85) --
	(119.87, 87.90) --
	(118.79, 90.89) --
	(117.51, 93.80) --
	(116.05, 96.63) --
	(114.42, 99.36) --
	(112.62,101.98) --
	(110.65,104.48) --
	(108.53,106.85) --
	(106.27,109.08) --
	(103.86,111.16) --
	(101.33,113.08) --
	( 98.69,114.84) --
	( 95.93,116.43) --
	( 93.08,117.85) --
	( 90.15,119.07) --
	( 87.15,120.11) --
	( 84.08,120.96) --
	( 80.97,121.61) --
	( 77.82,122.07) --
	( 74.65,122.32) --
	( 71.48,122.37) --
	( 68.30,122.22) --
	( 65.14,121.86) --
	( 62.01,121.31) --
	( 58.92,120.56) --
	( 55.88,119.62) --
	( 52.91,118.48) --
	( 50.02,117.16) --
	( 47.22,115.66) --
	( 44.52,113.99) --
	( 41.93,112.14) --
	( 39.46,110.14) --
	( 37.12,107.98) --
	( 34.93,105.68) --
	( 32.89,103.24) --
	( 31.00,100.68) --
	( 29.28, 98.01) --
	( 27.74, 95.23) --
	( 26.37, 92.36) --
	( 25.19, 89.41) --
	( 24.20, 86.39) --
	( 23.40, 83.31) --
	( 22.80, 80.19) --
	( 22.39, 77.03) --
	( 22.19, 73.86) --
	( 22.19, 70.68) --
	( 22.39, 67.51) --
	( 22.80, 64.35) --
	( 23.40, 61.23) --
	( 24.20, 58.15) --
	( 25.19, 55.13) --
	( 26.37, 52.18) --
	( 27.74, 49.31) --
	( 29.28, 46.53) --
	( 31.00, 43.86) --
	( 32.89, 41.30) --
	( 34.93, 38.86) --
	( 37.12, 36.56) --
	( 39.46, 34.40) --
	( 41.93, 32.40) --
	( 44.52, 30.55) --
	( 47.22, 28.88) --
	( 50.02, 27.38) --
	( 52.91, 26.06) --
	( 55.88, 24.92) --
	( 58.92, 23.98) --
	( 62.01, 23.23) --
	( 65.14, 22.68) --
	( 68.30, 22.32) --
	( 71.48, 22.17) --
	( 74.65, 22.22) --
	( 77.82, 22.47) --
	( 80.97, 22.93) --
	( 84.08, 23.58) --
	( 87.15, 24.43) --
	( 90.15, 25.47) --
	( 93.08, 26.69) --
	( 95.93, 28.11) --
	( 98.69, 29.70) --
	(101.33, 31.46) --
	(103.86, 33.38) --
	(106.27, 35.46) --
	(108.53, 37.69) --
	(110.65, 40.06) --
	(112.62, 42.56) --
	(114.42, 45.18) --
	(116.05, 47.91) --
	(117.51, 50.74) --
	(118.79, 53.65) --
	(119.87, 56.64) --
	(120.77, 59.69) --
	(121.47, 62.79) --
	(121.97, 65.93) --
	(122.27, 69.09) --
	(122.37, 72.27);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 72.27, 72.27) --
	( 36.84,107.70);

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 48.56, 87.69) {$\sqrt{t_0}$};
\end{scope}
\end{tikzpicture}


==> tikzR/rowVectors/shift_e1.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 72.27) -- (216.81, 72.27);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 70.46) --
	(216.81, 72.27) --
	(213.68, 74.08);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,  0.00) -- ( 72.27,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.08,213.68) --
	( 72.27,216.81) --
	( 70.46,213.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.58, 60.53) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 78.27,202.95) {$\mathbb{R}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 72.27, 72.27) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 83.11,119.25) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 28.91,155.38) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 72.27, 60.53) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 89.11,116.95) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 28.91,161.38) {3};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27, 72.27) --
	( 83.11,119.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 83.11,119.25) --
	( 28.91,155.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 28.91,155.38) --
	( 72.27, 72.27);
\end{scope}
\end{tikzpicture}


==> tikzR/rowVectors/shift_onevec.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 72.27) -- (216.81, 72.27);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 70.46) --
	(216.81, 72.27) --
	(213.68, 74.08);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,  0.00) -- ( 72.27,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.08,213.68) --
	( 72.27,216.81) --
	( 70.46,213.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.58, 60.53) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 78.27,202.95) {$\mathbb{R}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 83.11, 28.91) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 93.95, 75.88) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 39.75,112.02) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 83.11, 17.17) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 99.95, 73.59) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 39.75,118.02) {3};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 83.11, 28.91) --
	( 93.95, 75.88);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 93.95, 75.88) --
	( 39.75,112.02);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 39.75,112.02) --
	( 83.11, 28.91);
\end{scope}
\end{tikzpicture}

